F-RNG: Feed-Forward Relightable Neural Gaussians

Capturing relightable 3D assets from real-world objects is a widely researched problem. Several per-scene optimization-based methods, based on 3D Gaussian splatting (3DGS), support relighting; however, they usually require dense input views, and their overfitting nature makes it difficult to generalize across scenes. Unlike per-scene optimization methods, generalized feed-forward models can directly reconstruct Gaussians from sparse input views. However, the resulting assets have baked-in illumination and cannot be easily used for relighting. In this paper, we present F-RNG, a feed-forward framework that directly generates relightable 3DGS assets from sparse-view inputs. Training such a model from scratch can require massive data and computing resources, and it is especially challenging to generate relightable assets in a feed-forward manner with acceptable cost. We develop F-RNG upon an existing large reconstruction model (LRM) to extract relightable representations, while also utilizing priors from an intrinsic decomposition model (IDM). Specifically, we first introduce a latent-interpolated fine-grained geometry synthesis to enhance the LRM's geometry representation. Second, we propose a prior-guided relightable appearance distillation to extract relightable neural representations by incorporating IDM priors. Finally, a universal neural renderer enables flexible and high-fidelity relighting. F-RNG requires neither re-training nor fine-tuning of the underlying LRMs, thus can automatically benefit from better LRMs and IDMs in the future. With only small networks that can be trained with affordable data and computational resources, F-RNG avoids the repetitive inference of large models under different light conditions. By comparison to the state-of-the-art LRM-based relighting method, F-RNG achieves ~25x faster relighting, as well as superior quality (~+2.0 dB).

==> tables/knn.tex <==
\begin{table}[t]
\centering
\caption{ \textbf{\added{Robustness evaluation against global noise ratio and local perturbation intensity.}} Noise is introduced into Gaussian attributes (xyz, scale, and rotation). Specifically, global noise involves randomly perturbing attributes of a certain percentage of Gaussians across the entire scene, while local noise applies varying levels of perturbation to all Gaussians within a specific 20\% spatial region. The results demonstrate that our method, empowered by the KNN-based matching strategy, maintains superior stability under increasing interference levels compared to the baseline. When applying random Gaussian noise (std=0.02) to 20\% Gaussians of an object, LaMP-RNG outperforms RelitLRM with +0.5dB in PSNR, compared to -0.3dB (when without noise).} 
\label{tab:robustness}
\begin{tabular}{l c c c c c}
\toprule
\textbf{Setting} & \textbf{Method} & \textbf{0\%} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%}  \\ 
\midrule
\multirow{2}{*}{\shortstack{Global Noise }} & RelitLRM & \textbf{32.71} & 32.01 & 31.41 & 31.11  \\
 & \textbf{Ours} & 32.46 & \textbf{32.21} & \textbf{31.91} & \textbf{31.59}  \\
\midrule
\textbf{Setting} & \textbf{Method} & \textbf{0\%} & \textbf{5\%} & \textbf{10\%} & \textbf{20\%}  \\ 
\midrule
\multirow{2}{*}{\shortstack{Local Noise }} & RelitLRM & \textbf{32.71} & \textbf{32.26} & 31.76 & 31.25  \\
 & \textbf{Ours} & 32.46 & 32.13 & \textbf{31.96} & \textbf{31.65}  \\
\bottomrule
\addlinespace[0.5ex]
\multicolumn{6}{l}{\footnotesize}
\end{tabular}
\end{table}

==> tables/speed.tex <==
\begin{table}[htb]
    \centering
    \caption{
    \textbf{Rendering speed comparison between RelitLRM~\cite{zhang2024relitlrm} and our method.}
    We report rendering time per frame (ms) and speed-up ratios. 
    }
    \label{tab:speed_compare}
    \resizebox{0.42\textwidth}{!}{
    \begin{tabular}{l|cc}
        \toprule
        Dataset & RelitLRM (ms) & Ours (ms) \\
        \midrule
        \textsc{BlenderKit} & - & - \\
        \textsc{TensoIR}~\cite{jin2023tensoir}  & 4929 & 155 \\
        \textsc{Objaverse}$^\dagger$ ~\cite{deitke2023Objaverse} & - & - \\
        \textsc{Orb} ~\cite{kuang2023stanfordorb} & 3552 & 123 \\
        \textsc{Owl}~\cite{Ummenhofer2024OWL}  & - & - \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/tbl_exp_ab2.tex <==
\begin{table}[t]
    \centering
    \small
    % \scriptsize
    % \fontsize{7.5pt}{11pt}\selectfont
    \caption{ \textbf{Ablation on probabilistic design}. We design a deterministic counterpart by removing the noisy image tokens and keep the model architecture and training configuration the same. We compare our probabilistic design with the deterministic counterpart on our holdout evaluation set. 
    % \TYZ{Might remove the last two rows of 8 input views. The point we use diffusion is not to get  a higher PSNR, is that we can render specular objects much better.  }
    }
    \label{tbl:exp_determin}
    \begin{tabular}{lcccc}
    \toprule
          &  Input Views & PSNR & SSIM & LPIPS   \\
      \midrule
      Ours(full) & 4 & 27.63  & 0.922& 0.064   \\
      \midrule
      Ours(w/o. SH) & 4 & 27.10  & 0.912 & 0.076   \\
      \midrule
    \bottomrule
      % Ours over Single view & 81.0\% & 86.0\%
    \end{tabular}
    % \aftertab
\end{table}

==> tables/vs_l.tex <==
\begin{table*}[htb]
    \centering
    \caption{\textbf{Real world experiments.} Quantitative comparison on \textsc{Stanford-ORB} and \textsc{Objects-with-Lighting} datasets. We report PSNR-H, PSNR-L, SSIM, and LPIPS for Stanford-ORB, and PSNR, SSIM, and LPIPS for Objects-with-Lighting. The runtime and number of input views are also provided for each method.}
    \label{tab:real_world}
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{\textsc{Stanford-ORB}} & \multicolumn{3}{c|}{\textsc{Objects-with-Lighting}} & \#Input& Render\\
        & PSNR-L $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ &  views& time\\
        \midrule
        Ours  & 31.52 & 0.969 & 0.032 & 23.08 & 0.79 & 0.284 & 6 & 2 s\\
        \midrule
        RelitLRM & 33.26 & 0.979 & 0.023 & N/A & N/A & N/A & 42–67 & ?\\
        LightSwitch & 33.26 & 0.979 & 0.023 & N/A & N/A & N/A & 42–67 & ?\\
        \midrule
        DiffusionRenderer & 33.26 & 0.979 & 0.023 & N/A & N/A & N/A & 42–67 & ?\\
        DiLightNet & 33.26 & 0.979 & 0.023 & N/A & N/A & N/A & 42–67 & ?\\
        Neural Gaffer & 33.26 & 0.979 & 0.023 & N/A & N/A & N/A & 42–67 & ?\\
        
        \bottomrule
    \end{tabular}
    }
\end{table*}

